Unlocking Hardware Security Assurance: The Potential of LLMs

System-on-Chips (SoCs) form the crux of modern computing systems. SoCs enable high-level integration through the utilization of multiple Intellectual Property (IP) cores. However, the integration of multiple IP cores also presents unique challenges owing to their inherent vulnerabilities, thereby compromising the security of the entire system. Hence, it is imperative to perform hardware security validation to address these concerns. The efficiency of this validation procedure is contingent on the quality of the SoC security properties provided. However, generating security properties with traditional approaches often requires expert intervention and is limited to a few IPs, thereby resulting in a time-consuming and non-robust process. To address this issue, we, for the first time, propose a novel and automated Natural Language Processing (NLP)-based Security Property Generator (NSPG). Specifically, our approach utilizes hardware documentation in order to propose the first hardware security-specific language model, HS-BERT, for extracting security properties dedicated to hardware design. To evaluate our proposed technique, we trained the HS-BERT model using sentences from RISC-V, OpenRISC, MIPS, OpenSPARC, and OpenTitan SoC documentation. When assessedb on five untrained OpenTitan hardware IP documents, NSPG was able to extract 326 security properties from 1723 sentences. This, in turn, aided in identifying eight security bugs in the OpenTitan SoC design presented in the hardware hacking competition, Hack@DAC 2022.

==> Algorithm/Alg2.tex <==
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[t!]
%\begin{spacing}{0.9}
\vspace{0.7mm}
\raggedright{\textbf{Input}: ${\cal{R}}_a$, ${\cal{IP}}_A$}\\
%\vspace{0.5mm}
\textbf{Output}: $[{\cal{R}}_m]$
 \caption{Register Scan and Assemble for each Module}
%\end{spacing}
\vspace{1mm}
\textbf{\textit{Register Scan}(${\cal{R}}_a$, ${\cal{IP}}_A$)}
\begin{algorithmic}[1]
\State \textbf{Initialize} $[{\cal{R}}_m]'$, $[{\cal{R}}_m]$, \textbf{append} $[{\cal{R}}_m]$ $\leftarrow$ ${\cal{R}}_a$
\While{$[{\cal{R}}_{m}]'$ $!=$ $[{\cal{R}}_m]$}, 
\State $[{\cal{R}}_{m}]'$ $<=$ $[{\cal{R}}_m]$
\For {each ${\cal{A}}$ in [${\cal{A}}$] of ${\cal{IP}}_A$}
\If{${\cal{R}}_{i}$ in ${\cal{A}}$ and ${\cal{R}}_{x} \in [{\cal{R}}_m]$ in ${\cal{A}}$}
\State \textbf{append} $[{\cal{R}}_m]$ $\leftarrow$ ${\cal{R}}_i$
\EndIf
\EndFor
\EndWhile
\State \textbf{Return} $[{\cal{R}}_m]$
\end{algorithmic}
\label{algo:2}
\end{algorithm}

==> Background.tex <==
In this section, we will provide some background on hardware security verification, NLP, and the SoC designs used for developing the proposed NSPG tool.


\subsection{Hardware Security}

A plethora of techniques have been developed to ensure the security of software applications, either through the source code or binary operations~\cite{dessouky2019hardfails}. 
However, availability of commercial EDA tools, which are specifically crafted for hardware security, is rare.
%\textcolor{orange}{However, few Electronic Design Automation (EDA) tools, which are specifically crafted for hardware security, are commercially available~\cite{dessouky2019hardfails}. 
Hence, recently, researchers have focused on developing tools and methodologies to ensure hardware security. We will provide a background of recent hardware security verification approaches as well as hardware design documentation in the following subsections.

% The software industry has introduced several tools and methodologies for evaluating the security robustness of the software, either for source code or for binaries~\cite{dessouky2019hardfails}.
\subsubsection{Hardware Security Verification Approaches}



\textbf{Information Flow Tracking (IFT)}: \textcolor{black}{Information Flow Tracking improves hardware security by identifying malicious input interfaces, regulating the use of counterfeit information, and verifying hardware operation flows~\cite{suh2004secure, tiwari2009complete, oberg2010theoretical, ardeshiricham2017register, qin2020formal, ardeshiricham2019verisketch}.} Although this approach can effectively detect malicious attacks, its performance is not guaranteed when evaluating complex RTL designs systematically without security properties.
\smallskip

\noindent\textcolor{black}{\textbf{Theorem Proving}: Theorem proving utilizes a language, VeriCoq, to automate the transformation of RTL into Coq theorem. This approach validates (proves) the converted language through the Proof-Carrying Hardware Intellectual Property (PCHIP) framework and ensures the robustness of a third party IP with formal proofs of security properties~\cite{love2011proof,bidmeshki2015vericoq}. 
Although theorem proving provides a sufficient verification method for CPUs, its efficiency on complex RTL relies on appropriate security properties.}
\smallskip

\noindent\textbf{Assertion-based Verification}: Assertion-based security verification employs formal and simulation-based methods to detect violations against assertions included in RTL designs~\cite{bilzor2012evaluating, hicks2015specs}. Assertions are created via analysis of the security properties, which protect the integrity of the system. While this approach has been successfully applied to SoC cores, it might not be fully scalable when applied to non-core components, such as peripherals~\cite{zhang2020transys, farzana2019soc}.
\smallskip

\noindent\textbf{Property Specific Information Flow}: This technique utilizes property specifications to generate information flow models that are catered to the pre-defined security properties. The models are verified by conducting a property-specific search and identifying security-critical paths~\cite{hu2018property}. The security properties can be used to generate constraints, which define the operation behaviors and register values. \textcolor{black}{Formal verification methods, such as Security Path Verification (SPV), utilize security properties to identify malicious information flows that require design inspections~\cite{JasperGo88:online}.}

\smallskip

%\vspace{0.1in}
\noindent\textbf{Symbolic testing}: Since formal approaches usually cause state space explosion, directed test generation has been developed to address this issue. Existing researches, such as~\cite{ahmed2018directed, lyu2020automated}, utilize control flow graphs on RTL models to ensure functional correctness. However, they have not considered the application of security properties in their algorithms and therefore fail to detect vulnerabilities. On the other hand, techniques incorporating security properties and concolic testing were able to detect violations in RTL and conclusively verify the design~\cite{meng2021rtl, zhang2018end}. %Furthermore, they accounted for corner cases and were associated with significantly lower overhead.

In summary, all existing security verification techniques need robust security properties to ensure the trustworthiness and robustness of the RTL. Therefore, in order to comprehensively validate the entire SoC, we require an effective security property generation technique that provides design assertions or operating constraints. %Hence, the lack of efficient security properties is usually the bottleneck to most hardware security verification approaches.

\subsubsection{Hardware Design Documentation}

% Due to the size of embedded systems and the reuse of components, well-crafted documentation of software and hardware is needed to strengthen the understandability of the application.
\textcolor{black}{In order to enhance the comprehensibility of the SoCs, it is imperative to have access to thorough documentation of \textcolor{black}{SoCs}, considering their complexity and dependence on reusable components}. However, their documentation is commonly considered providing limited value for any scientific analysis. Therefore, little effort has been put into subjects related to any hardware documentation analysis. %Furthermore, more attention are focuse development is usually considered as much more important than system documentation, and the documentation of the system is mentioned only briefly~\cite{keating2002reuse}.
%Meanwhile, existing documentation for the latest version of the project is usually incomplete and often too complicated for systemic analysis. 
\textcolor{black}{In reality, technical documentation is an important part of the overall product and should be prioritized along with the design and implementation stages. In more than one instance, insufficient documentation has been regarded as the major reason for design failure~\cite{bentley2001validating}.}
Therefore, hardware designs, such as RISC-V and OpenTitan, document hundreds of pages for Industry Standard Architecture (ISA) and non-ISA specifications.
Additionally, various tools have been introduced to generate system documentation more efficiently. {For instance, ``Javadoc'' provided by Sun Microsystems generates API documentation in HTML from the comments in the source code, and ``CppDoc'' generates HTML for automatic source code documentation~\cite{JavadocT88:online, GitHubsh47:online}.}
Therefore, these tools can provide us with more opportunities to systematically analyze hardware design documents and generate security properties from them.
% These provide us an opportunity to systematically analyze the hardware design documents provided by the hardware design foundations and generate security properties from them.
%\begin{comment}
\subsubsection{Hardware Security Property}

The specification of security properties usually varies from the method of security analysis, producing specifications that are unique to the selected verification tools or models~\cite{mana2008towards}. 
\begin{center}
\begin{minipage}{0.95\linewidth}
\vspace{-0.1in}
\begin{lstlisting}[caption={Security Property and SystemVerilog Assertion},label={lst:1}, escapechar = @]
Security Property Description:
If the AES unit wants to finish the encryption/decryption of a 
data block but the previous output data has not yet been read by 
the processor, the AES unit is stalled.

SystemVerilog Assertion:
assert 
    property (                                  
        @\@@(posedge clk) disable iff (rst)    // Security Property
        aes.done |-> aes.out @==@ @\$@past(aes.key)
        )
        else                                // Error Message
            @\$@error("@\%@m previous key has not been read");
\end{lstlisting}
\end{minipage}
\end{center}
Listing~\ref{lst:1} shows an example of SystemVerilog Assertion based on the description of the security property. It shows that in order to generate an appropriate term for verification mechanism, the descriptions of security properties must contain strong reasoning and details of the operation.
For example, Listing~\ref{lst:1} shows a paragraph from OpenTitan AES document. The sentences marked in blue are security property-related ones, and the rest are unrelated.

\begin{center}
\begin{minipage}{0.95\linewidth}
\vspace{-0.1in}
\begin{lstlisting}[caption={A example paragraph in AES Document},label={lst:2}, escapechar = @]
Also, there is a back-pressure mechanism for the output data. @\aftergroup\bluecolor@
If the AES unit wants to finish the encryption/decryption of a 
data block but the previous output data has not yet been read by 
the processor, the AES unit is stalled. @\aftergroup\blackcolor@It hangs and does not 
drop data. The order in which the output registers are read 
does not matter. @\aftergroup\bluecolor@Every output register must be read at least 
once for the AES unit to continue.@\aftergroup\blackcolor@ This is the default behavior. 
@\aftergroup\bluecolor@It can be disabled by setting the MANUAL_OPERATION bit in 
CTRL_SHADOWED to 1.@\aftergroup\blackcolor@
\end{lstlisting}
\end{minipage}
\end{center}

It is obvious that the security properties have more distinguished contexts compared to other regular sentences in the paragraph. Hence, it becomes possible for us to distinguish the security property-related sentences in any documentation since these sentences present precise definition of the semantics, key words of the processes, or relation between several operation factors.
Therefore, we can emphasize on these aspects when fine-tuning the language model by enhancing and identifying the security property-related context in each sentence.
The goal of our proposed technique is to extract these security property-related sentences from the rest of the documentation.
%\end{comment}


\subsection{OpenTitan Architecture and Threat Model}


\subsubsection{OpenTitan SoC Architecture}

Since we do not have access to commercial designs, our framework has been developed using open-source SoCs, such as RISC-V and OpenTitan.
In this work, RISC-V documentation is only used for training. OpenTitan documentation, on the other hand, is used for both training and validation. We obtained access to \textcolor{black}{the buggy OpenTitan design} in the Hack@DAC 2022 hardware hacking competition~\cite{HACKDAC211:online}. 
% since we have participate in the Hack@DAC 2022 hardware hacking competition, we have access to its buggy design~\cite{HACKDAC211:online}. 
\textcolor{black}{Figure~\ref{fig:opentitan} illustrates the design architecture of the open-source OpenTitan Earl Grey SoC used in the competition. Earl Grey features a low-power, secure microcontroller designed for security applications.} 
The block diagram displays the system configuration, including the Ibex processor and all memories and integrated circuits~\cite{OpenTita77:online}. It includes a 32-bit RV32IMBC RISC-V core with enhanced physical memory protection and various security features, such as dummy instruction insertion and dual-core lockstep configuration. Earl Grey also includes a range of ``peripherals'', or subservient execution units connected to the Ibex processor via a bus interconnect, including security peripherals and general-purpose I/O (GPIO) peripherals.
\textcolor{black}{The security peripherals consist of cryptographic modules, such as AES, Hash-based Message Authentication Code (HMAC), Keccak Message Authentication Code (KMAC), one time programmable (OTP) memory controller, Life Cycle (LC) Controller, a One Time-programmable Big Number accelerator for RSA and ECC (OTBN), and a NIST-compliant Cryptographically Secure Random Number Generator (CSRNG)}. The GPIO peripherals include multiple management system, such as clock, reset, power and frequency timer.

\begin{figure}[t!]
\centering
  \includegraphics[width=1\columnwidth]{Figure/Opentitan.png}
  \vspace{-0.1in}
  \caption{OpenTitan architecture. }
  \label{fig:opentitan}
  %\vspace{-0.1in}
\end{figure}


\input{Figure/framework.tex}

\subsubsection{Threat Model}
\label{sec:threat}

Our threat model is based on the one used in Hack@DAC 2022, which consists of the following attack scenarios:
 \begin{itemize}
     \item \textcolor{black}{An unprivileged software adversary that can access the core in user mode, with control over user-space interfaces and the ability to issue unprivileged system instructions and request feedback.}
    \item A privileged software adversary that can execute code with supervisor privilege but may target other higher privilege levels or bypass security countermeasures.
    \item An authorized debug adversary which is capable of unlocking and debugging production devices.
    \item \textcolor{black}{An adversary that has physical access to the hardware and is capable of adding or removing components, as well as debugging through the JTAG interface.}
    %\item 
 \end{itemize}
The aim of the adversary is to exploit any potential vulnerabilities in the SoC in order to bypass any security objective.

\subsubsection{Security Objectives and Features}
\label{sec:objective}

The security objectives of OpenTitan are as follows~\cite{HACKDAC211:online}:
\begin{itemize}
    \item \textit{\textbf{SO1}}: \textcolor{black}{Preventing privilege level compromise due to unprivileged code running in the core.}
    \item \textbf{\textit{SO2}}: Protecting system debug interface from malicious or unauthorized debugger.
    \item \textit{\textbf{SO3}}: Protecting device integrity and preventing exploits from a software adversary.
\end{itemize}
Various security features have been developed for the SoC to support the aforementioned security objectives, including privileged access control to peripherals, write and read locks on registers to protect the privilege integrity from unprivileged instruction, and domain reset to flush sensitive information in cryptographic processors. 
The details of the OpenTitan SoC for our experiments will be discussed in Section~\ref{sec:setup}.


\subsection{Natural Language Processing}

\textcolor{black}{Natural Language Processing (NLP) is a field of study that
focuses on applying computational techniques to understand,
learn, and generate human language content. Early researches in NLP concentrated on automating linguistic structure analysis and development of basic functionalities, such as automatic translation, and speech recognition and synthesis.} In recent times, the framework has been continuously refined and utilized in practical applications. \textcolor{black}{NLP plays a crucial role in various industries and has a wide range of applications, ranging from real-time translation and social media search engines to sentiment analysis~\cite{feng2021survey}.} %Figure~\ref{fig:NLPapp} shows the various applications of NLP. 
In this section, we will discuss the following facets of NLP that are integrated in NSPG.

%\begin{figure}[t!]
%\centering
%  \includegraphics[width=0.9\linewidth]{Figure/NLP_app.pdf}
  %\vspace{-0.1in}
%  \caption{Example of an NLP application.}
%  \label{fig:NLPapp}
  %\vspace{-0.1in}
%\end{figure}



\subsubsection{Bidirectional Encoder Representations from Transformers (BERT) Model}

Most state-of-the-art natural language models are built on transformer architectures, such as BERT, which are effective at modeling long-range dependencies in text~\cite{gillioz2020overview}. These models utilize a multi-layer, multi-head self-attention mechanism, which allows for efficient parallel computation on GPUs~\cite{devlin2018bert}. \textcolor{black}{First, the input token sequence is parsed by a lexical encoder by combining the token, position, and segment embedding, as shown in Figure~\ref{fig:SQ}. The resulting embedding is subsequently processed by the various layers of the transformer modules. Next, a contextual representation of each token comprising transformer layer $L$ is created by allocating weight values to the tokens belonging to layer $L-1$.} The token attentions are computed by using the current token's representation as the query. Lastly, the final layer provides the contextual representations for all tokens by combining the position, segment, and textual details from the entire input text sequence. \textbf{We build the NSPG framework based on the BERT model.}
\begin{figure}[tb!]
\centering
  \includegraphics[width=1\linewidth]{Figure/SQ_model.png}
  \vspace{-0.1in}
  \caption{BERT model tokenization.}
  \label{fig:SQ}
  %\vspace{0.1in}
\end{figure}

\begin{figure}[tb!]
\centering
  \includegraphics[width=1\linewidth]{Figure/BertModel.png}
  %\vspace{-0.1in}
  \caption{Mask language model.}
  \label{fig:BertModel}
  %\vspace{-0.1in}
\end{figure}



\subsubsection{Sequence Classification Model}

Sequence classification model (SCM) divides sequences into predefined sentiment categories~\cite{devlin2018bert}. It is a supervised machine-learning problem and can be either binary (positive or negative) or fine-grained (with multiple layers of scales). Given a text span and a category (such as an abstract or domain-specific text), the model aims to classify the text as belonging to the category or not. The text is first pre-processed by appending a [CLS] token that marks the beginning of the sequence and a [SEP] token that defines the end of the sequence. The content will be passed through a featurization step, typically using a BERT encoding, similar to the model shown in Figure~\ref{fig:SQ}. The resulting features are fed into a final classification layer, which is typically a simple linear layer. \textbf{Our proposed framework, NSPG, will apply this model to categorize each sequence of sentences and identify if they belong to security property or non-property descriptions in the documents.}

\subsubsection{Mask Language Model}

Masked Language Model (MLM) is a self-supervised learning method used in state-of-the-art BERT models, such as SciBERT or RoBERTa~\cite{beltagy2019scibert, devlin2018bert}. This language model is trained to predict a randomly masked subset of tokens in a given input sequence. During training, a certain percentage of tokens are randomly selected and replaced with a special token ([MASK] in BERT). The trained model will predict the original tokens based on the context provided by the remaining unmasked tokens, as shown in Figure~\ref{fig:BertModel}. \textcolor{black}{The primary objective is to minimize the cross-entropy loss between the predicted tokens and their original counterparts.} For instance, in SciBERT and RoBERTa, by default, 15\% of the input tokens are chosen for masking, with 80\% probability of being replaced by [MASK], 10\% left unchanged and 10\% randomly replaced by another token from the vocabulary~\cite{devlin2018bert}. The language model utilizes MLM to improve its ability to comprehend the context and relationships between each word in a sequence. This approach has proven to be effective in enhancing the performance of language models on various tasks, including language processing and machine translation. \textbf{We will utilize this model to further process the extracted sequences from the design document and generate appropriate security properties.}

%\begin{figure*}[tb!]
%\centering
%  \includegraphics[width=0.9\textwidth]{Figure/Bert_flow.png}
%  %\vspace{-0.2in}
%  \caption{Proposed Framework NSPA.}
%  \label{fig:bertflow}
  %\vspace{0.1in}
%\end{figure*}

\subsubsection{Data Augmentation}

Data augmentation (DA) is a method of enhancing the diversity of training data without collecting more data. It involves adding modified copies of existing data or creating synthetic data to act as a regularizer and reducing overfitting during the training of machine learning models~\cite{feng2021survey}. \textcolor{black}{However, since the input space in NLP is predominantly discrete, it is challenging to produce effective augmented data that captures the invariances.} Many DA techniques have been proposed for NLP, including rule-based manipulations and generative approaches. Ideal DA techniques should be easy to implement and further improve model performance. \textcolor{black}{Techniques that use trained models may be more expensive to implement. However, they introduce more variance in data, thereby resulting in enhanced model performance. Although model-based techniques are designed to boost performance in downstream tasks, they are difficult to develop and use. This may result in overfitting or performance degradation when trained on out-of-domain examples.} %Effective DA approaches should aim for balance. 
Overall, DA transformations can be recognized as kernels that help with the averaging of features and variance regularization. \textbf{Since this is the first work that mainly focuses on the design documentation of the hardware security domain, our data samples are limited to the open-source documentation; thus, we will apply different DA approaches and choose the best-performing approach regarding the hardware domain. The details will be discussed in Section~\ref{method}.}

==> Method.tex <==
\input{Table/table1.tex}
\label{sec:method}
Figure~\ref{fig:bertflow} presents our proposed approach, NSPG. The first step involves extracting security properties and non-property-related sentences from the hardware design documentation of OpenTitan and RISC-V. Next, we modify them using data augmentation and hardware domain-specific formalization to create an enhanced dataset for training the general BERT model. 10865 sentences from OpenTitan documentation are used for fine-tuning the mask language model. 
To validate the classification model, we generate training samples consisting of \textcolor{black}{4027 sentences (out of which 1891 are security \textcolor{black}{property-related} sentences and the rest are \textcolor{black}{non-property-related} sentences)} from the top module and test cases documentation in OpenTitan design, and privileged and non-privileged documentation for RISC-V. We also generate an additional 630 security property-related and non-property-related sentences from Analog-to-Digital Converter (ADC), and AES encryption module documentation in OpenTitan design, and tracing documentation from RISC-V design for validation. The modified and non-modified sample datasets are used to train the BERT model, and \textcolor{black}{the validation dataset is used to evaluate the performance of each trained sequence classification model}. In this work, we employ the SciBERT and general BERT model as our encoder and compare their performances~\cite{beltagy2019scibert} in Section~\ref{sec:bertcom}. The validation of the data augmentation and hardware domain-specific formalization processes will be described in detail in Section~\ref{sec:spg}.


\subsection{Data Modification and Enhancement}
\label{sec:datamod}
In order to improve the performance of the MLM and SCM with limited data samples, we will apply data augmentation to improve the sample size of the dataset for the MLM. Furthermore, we will utilize hardware domain-specific formalization to enhance the dataset for the sequence classification model.


\input{Table/table8.tex}


\subsubsection{Data Augmentation (DA)}

\label{sec:da}
DA is a key component for enhancing the quantity of the data samples, which involves generating two correlated views of a data point in order to increase the amount and diversity of training data. Although it is important to ensure the diversity of the generated data, the structure and semantics of the original sentence should not be modified. In NSPG, we focus on operation relations and structures in the sentences since most of the security properties involve the behaviors of two entities in the design. We capture the necessary information for the operating entities and apply DA to swap or replace the rest of the tokens in the sentence. The closest sentiment texts are provided by Wordnet, a large lexical database of English where synonyms are interconnected by means of conceptual-semantic, to generate the augmented data~\cite{miller1995wordnet}. We experimented with four techniques: random swap, random deletion, synonym replacement, and random insertion. These are the most common data augmentation technique available for NLP model~\cite{feng2021survey}. The tokens in the texts are modified in the following ways to generate the augmented data:
\begin{itemize}
    \item \textbf{Random Swap (RS)}. We exchange the positions of two randomly selected phrases such as nouns and conjunctions while maintaining the operation behavior and structure of the original sentence. 
    \item \textbf{Random Deletion (RD)}. In order to keep the original context, we randomly delete one of the adjectives, determiners, or adverbs in the sentence.
    \item \textbf{Synonym Replacement (SR)}. We randomly replace verbs in the sentence with their closest synonyms obtained from the WordNet database. 
    \item \textbf{Random Insertion (RI)}. We summarize all the adverbs that are used in the documentation and \textcolor{black}{randomly select one to insert into the sentence near verbs}.
\end{itemize}
Table~\ref{tab:DA} presents examples of these techniques applied to a sentence from the DA task. Random Swap takes parts of the sentence ``when in this mode'', and places them into a random spot of the sentence, which is at the end of the sentence. On the other hand, Random Deletion removes the definition term in the sentences such as ``some'' in the sentence. 
Synonym Replacement utilizes the Wordnet database to replace the verb in the sentence, such as ``occur'', with its sentiment ``happen''.
Random Insertion randomly chooses the most common adverb used in the documents such as ``immediately'', and places them before or after the verb in the sentence. Each method tends to introduce diversity in the original sentence, and increase possible word usage, thereby reducing data overfitting and boosting the generalization ability of the model. \textcolor{black}{
We train four BERT MLM models using different augmented data (in combination with the original data from the documentation) and evaluate their performance to determine the best model.} The details will be discussed in Section~\ref{sec:spg}.

\begin{figure*}[tb!]
\centering
  \includegraphics[width=0.95\textwidth]{Figure/reconstruct.png}
  %\vspace{-0.1in}
  \caption{Sentence formalization in documents. The first row represents the original sentence in the document. The second row shows each fragment of the original sentence. The third row demonstrates the process of reconstructing the missing components of each fragment, and the last row shows the sentence after constructing the missing components.}
  \label{fig:reconstruct}
  \vspace{-0.1in}
\end{figure*}

\subsubsection{Data Pre-Processing and Sentence Formalization}
\label{sec:sefor}

\textcolor{black}{Data pre-processing and data cleansing are utilized to generate unbiased data, which in turn is critical to furnish reliable machine learning algorithms~\cite{felix2019systematic}.} %Studies have shown that biased learning can result from training on imbalanced or noisy data~\cite{stefanowski2016dealing, krawczyk2014cost}.
Studies have shown that biased learning can result from training on imbalanced or noisy data~\cite{stefanowski2016dealing, krawczyk2014cost}. Therefore, significant consideration should be provided to the data cleansing process and detailing the methods used in our studies. BERT model tokenizer is used to tokenize the sentences by its data pre-processing technique~\cite{devlin2018bert}.
In NSPG, in order to improve the performance
for sequence classification, we propose a hardware domain-specific formalization to further differentiate the feature of each sentence in the documents, which enforces the BERT model to recognize more contextual semantic information and dependencies. For instance, texts or sentences related to hardware operations and behavior are considered in-domain, while descriptions of the document are regarded as out-domain.

Although a plethora of data pre-processing techniques have been proposed to improve the performances of machine learning techniques in text mining and image classification~\cite{gupta2017set, iliou2015novel}, there have been few studies pertaining to NLP.
In this work, we consider some data pre-processing methods with hardware security-domain modification and validate their impact on model performances. 
As shown in Table~\ref{tab:preprocess}, we apply several alternative methods, including noun swapping, verb swapping, fragment deletion, and fragment insertion, to preprocess each sentence in the dataset. 
Noun swapping intends to remove the arbitrary term used in each sentence, such as KEYMGR, and replace them with more generalized terminology in the hardware domain. 
Verb swapping substitutes the verbs in the sentence with sentimental hardware domain-related verbs.
\textcolor{black}{Fragment removal deletes parts of the sentence while retaining the more essential content of hardware operations.}
Fragment addition adds information to the incomplete sentence, constructing each fragment of the sentence with a similar structure.
Among these approaches, only fragment addition improves the performance of the classification model. While noun swapping and verb swapping do not significantly affect performance, fragment removal degrades performance.
Thus, we can infer that instead of utilizing pre-processing to simplify the data, the NLP model tends to require more information and complete structure in each sentence to learn the subjects more accurately. Intuitively, the prevailing assumption is that using more in-domain text in the training datasets should help with domain-specific classification.
Although each sentence in the document is constructed differently, we will explore this concept by adding domain-specific portions for each sentence. %\textit{e.g.}, the nouns and verbs in the sentence.

Figure~\ref{fig:reconstruct} shows an example of formalizing a sentence in the document. First, we break the sentence ``When resetting, if 0, allow requests to pass through the host-side FIFO with no clock delay.'' into fragments by identifying each conjunction ``When'', ``if'', and ``to'' in the sentence, and separating the sentence into fragments as ``When resetting'', ``if 0'', ``allow requests'', and ``to pass through the host-side FIFO with no clock delay''. In these fragments, ``When resetting'', and ``allow requests'' are missing nouns, ``if 0'' is missing noun and verb, and ``to pass through the host-side FIFO with no clock delay'' is complete. We will add these missing components into the fragments by applying the trained mask language model and placing appropriate terms into the fragments. Hence,  ``When resetting'', ``if 0'', and ``allow requests'' will be transformed into ``When system is resetting'', ``if value is set 0'', and ``module allows requests''. We train BERT sequence classification model with different combinations of the original and formalized training datasets to evaluate the classification performance based on accuracy, recall, precision, and F1-score, which are defined as follows. 
% \vspace{-0.1in}
%\begin{adjustbox}{width=\columnwidth,center}
{\small
\begin{gather}
    Accuracy = \frac{True\, Positives + True\, Negatives}{All\, Prediction} \\  Recall = \frac{True\, Positives}{True\, Positives + False\, Negatives} \\ Precision = \frac{True\, Positives}{True\, Positives + False\, Positives} \\ F1-Score = 2*\frac{Recall*Precision}{Recall + Precision}
\end{gather}
%\end{adjustbox}
}%
%\vspace{-0.1in}
In the above formulae, True Positives refer to the correctly extracted security properties. False Negatives refer to the security properties that are not extracted from the documents. On the other hand, False Positives refer to the non-property sentences extracted by the framework. Finally, True Negatives correspond to the correctly identified non-property sentences. Accuracy demonstrates the classification performance of the framework, \emph{i.e.}, how well it can distinguish between property and non-property sentences. Recall and precision indicate the fraction of false negative and false positive classifications made, respectively. F1-score represents the general performance of a classification model in terms of recall and precision.
% In order to generate as many security properties as possible potential properties, a few non-property-related sentences are tolerable and can be removed with further analysis.
Since our priority is to maximize the generation of security properties, we can tolerate the presence of a few non-property-related sentences (\emph{i.e.}, False Positives), which can be removed with further analysis. Therefore, accuracy and recall are the key information to determine the performance of sentence formalization and SCM in NSPG. Higher values of accuracy and recall indicate better performance of the formalization method and SCM model. The details will be discussed in Section~\ref{sec:trsec}.


\subsection{Security Property Generation}
\label{sec:spg}
\input{Algorithm/Alg1.tex}
In this section, we will explain the process of security property generation from the design documents. Figure~\ref{fig:secgen} illustrates the training procedure of NSPG, which consists of three stages. In the first stage, we will train the MLM with unlabeled data from hardware design documentation. In the second stage, we will modify extracted security properties with the MLM to fine-tune SCM. Lastly, we will utilize the fine-tuned SCM to generate security properties from the documents. Algorithm~\ref{algo:1} demonstrates the details of each stage for the training and security property generation process.

%First, the MLM will be trained with unlabeled documentation to comprehend the specific domain. Second, we will utilize the trained MLM to construct the labeled dataset regarding the registers and their operation information. Further, we will use the enhanced labeled dataset to train the SCM, and categorize each sentence in the unseen documents into property and non-property. Figure~\ref{fig:secgen} illustrates the training procedure of NSPA, which consists of three stages. In the first stage, we will train the MLM with unlabeled data from hardware design documentation. In the second stage, we will modify manually extracted security properties with the MLM to finetune sequence classification model. Lastly, we will utilize the finetuned SCM to generate security properties from the documents. Algorithm~\ref{algo:1} demonstrates the details of each stage for the model training and security property generation process.

\begin{figure}[tb!]
\centering
  \includegraphics[width=0.9\linewidth]{Figure/Sec_Gen.png}
  %\vspace{-0.1in}
  \caption{BERT model training process.}
  \label{fig:secgen}
  %\vspace{0.1in}
\end{figure}

%\input{Algorithm/Alg1.tex}

\subsubsection{General BERT vs SciBERT model}
\label{sec:bertcom}
\input{Table/table7.tex}

In this section, we will discuss two popular BERT models and motivate our choice for inclusion of one on NSPG.
General BERT utilizes WordPiece~\cite{wu2016google} for unsupervised tokenization of input sequences, building its vocabulary with the most frequently used words or sub-word units. SciBERT, on the other hand, is constructed with a new WordPiece vocabulary on a scientific corpus using the SentencePiece1 library~\cite{sennrich-etal-2016-neural}. The token overlap between BERT and SciBERT vocabulary is 42\%, indicating a substantial difference in the frequently used words between scientific and general domain texts. {SciBERT was trained on a dataset comprising 1.14M papers from Semantic Scholar, where 82\% of the papers belong to the biomedical domain, while the remaining 18\% pertain to computer science~\cite{ammar2018construction}.}

Table~\ref{tab:BERTvs} shows the comparison between general BERT and SciBERT, using the same data modification method and the same labeled dataset with 2000 samples. FT refers to formalized training data only, FTT refers to formalized training and testing data, and FTO refers to formalized training data with original training data. FTOT refers to formalized training and testing data with original training data. \textcolor{black}{The results indicate that both BERT models show improved performance in comparison to their base models, with an average increase of 0.6\% accuracy with General BERT and 3.4\% accuracy with SciBERT.} For each data modification method, the largest effects of fine-tuning were observed in the FTO (+5.9\% accuracy with SCIBERT and +2.9\% accuracy with General BERT) and FTOT (+4.9\% accuracy with SciBERT and +0.1\% accuracy with General BERT). While little effect was seen on recall, precision, and F1-score for SciBERT, General BERT sees a significant improvement in recall when applying FTO (+15.4\%). However, SciBERT, with fine-tuning, outperforms General BERT on accuracy and recall, while performing similarly on precision and F1-score. \textcolor{black}{Based on these observation, we determine that SciBERT is more suitable for extracting all potential security properties, which we have subsequently incorporated in NSPG.}


\subsubsection{Training Mask Language Model (MLM)}
\label{sec:mlm}
The purpose of MLM is to understand the detail of each sentence demonstrated in the document and predict the masked content. Hence, we will select the model having the lowest perplexity and loss, which indicates that the model has the best comprehension of the hardware domain and the best prediction of each sample, respectively. Each model is trained with samples from the OpenTitan and RISC-V documentation, which consists of 10865 sentences and additional data from the DA task.
\textcolor{black}{Table~\ref{tab:mlm} shows the training loss, training runtime, perplexity, and sample sizes for each DA approach, as described in Section~\ref{sec:da}. As shown in the table, the DA task significantly increases the sample size and improves the performance of the MLM model, and Random Insertion (RI) operation performs the best among all four tasks with a perplexity score of 5.} Therefore, we use the MLM model trained with data from RI for our further process flows. 

%\begin{minipage}{0.5\textwidth}


\input{Table/table2.tex}

%\input{Algorithm/Alg1.tex}

\input{Table/table3.tex}

%\end{minipage}

\subsubsection{Training Sequence Classification Model (SCM)}
\label{sec:trsec}
In this stage, NSPG will separate the content in the documents according to the labeled dataset.
In order to simulate the scenario in which the SCM is applied on an unseen document to determine whether the sentence is a security property or not, we will test each trained sequence classification model on a validation dataset. This dataset consists of 470 extracted security properties and non-properties from OpenTitan AES and ADC documentation, and 160 from RISC-V trace documentation.
\textcolor{black}{Table~\ref{tab:SC} shows the results for the data modification approach, as described in Section~\ref{sec:sefor}. The SciBERT model trained with the FTO modification performs the best with an average of 80.3\% accuracy, 91.5\% recall, and 85\% F1-score. \textcolor{black}{Since this modification method consists of both the original and the formalized sentences, it improves the diversity of the training dataset, which helps the model to learn more features of a property-related sentence.} Hence, we will use this method as our final pre-processing method for the SCM model.} 

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\subsubsection{Security Property Generation}

After validating each procedure in training, we will construct the pipeline of the BERT model training process, utilize the classification model to analyze the unseen documents, and extract the security properties which contain information about operation behavior, and register interaction. %However, the extracted sentence might provide incomplete information regarding the security properties. Therefore we need to further complete the content of the sentence. For example, an extracted sentence such as ``Once firmware initialization is complete, it is important to exit this mode if the endpoints ever need FIPS-approved random values.'' lacks the information of ``this mod''. However, it is mentioned in the document, where ``this mod'' is referring to ``Boot-time Request Mode'' (BOOT\_REQ\_MODE). We will capture this information from the register checklist in the document, and try to replace ``this mode'' with register information which is ``BOOT\_REQ\_MODE''. Hence, the final generated security property will be presented as ``Once firmware initialization is complete, it is important to exit BOOT\_REQ\_MODE if the endpoints ever need FIPS-approved random values.'', which contains both the registers and the required operation.
We will evaluate the extraction process and examine the SoC with the extracted security properties, as discussed in Section~\ref{experiment}.% and Section~\ref{discussion}.




==> SoC_Objective.tex <==


\begin{figure*}[tb!]
\centering
  \includegraphics[width=0.80\textwidth]{Figure/Opentitan.png}
  %\vspace{-0.2in}
  \caption{Opentitan Architecture. }
  \label{fig:opentitan}
  %\vspace{0.2in}
\end{figure*}

\subsection{Opentitan SoC Architecture}

In this work, RISC-V documentation will be only used for training. We will use the Opentitan documentation for both training and validation since we have the access to its buggy design in the Hack@DAC 2022. 
Figure~\ref{fig:opentitan} shows the high-level architecture of the open-source Opentitan Earl Grey SoC used in the Hack@DAC 2022 hardware hacking competition~\cite{HACKDAC211:online}. Earl Grey is a low-power, secure microcontroller designed for use cases requiring hardware security. The block diagram displays the system configuration, including the Ibex processor and all memories and integrated circuits~\cite{OpenTita77:online}. It includes a 32-bit RV32IMBC RISC-V core with enhanced physical memory protection and various security features, such as dummy instruction insertion and dual-core lockstep configuration. Earl Grey also includes a range of ``peripherals'', or subservient execution units connected to the Ibex processor via a bus interconnect, including security peripherals and general-purpose I/O (GPIO) peripherals. The security peripherals consist of cryptographic modules such as AES, HMAC, KMAC, a programmable big number accelerator for RSA and ECC (OTBN), and a NIST-compliant cryptographically secure random number generator (CSRNG). The GPIO peripherals include a clock, reset and power management, a fixed-frequency timer, and an always-on timer. The entire SoC documentation comprises 33 IP design specifications with approximately 12000 sentences. Each IP design documentation includes information on register descriptions, functionalities, and operation processes. Among these, the content of operation processes can be transformed into security properties, which we label as security properties and the rest as non-property sentences.


\subsection{Adversary and Threat Model}

Our security threat model consists of four attack scenarios, as follows:
 \begin{itemize}
     \item An unprivileged software adversary that can execute code on the core in user mode, with control over user-space processes and the ability to issue unprivileged instructions and system calls.
    \item A privileged software adversary that can execute code with supervisor privilege but may target other higher privilege levels or bypass security countermeasures.
    \item Authorized debug adversary which is capable of unlocking and debugging production devices.
    \item A hardware adversary that has physical access to the device and can add or remove components, as well as possessing the skills of a JTAG debugger.
    %\item 
 \end{itemize}
The aim of the adversary is to exploit vulnerabilities in the system in order to bypass security objectives and invoke unintended functionality.


\subsection{Security Objectives and Features}

\input{Table/table4.tex}

Several security objectives of the SoC are specified in the competition, and we will utilize them in our work:
\begin{itemize}
    \item \textit{\textbf{SO1}}: Preventing unprivileged code running in the core from compromising privilege level.
    \item \textbf{\textit{SO2}}: Protecting system debug interface from malicious or unauthorized debugger.
    \item \textit{\textbf{SO3}}: Protecting device integrity and preventing exploits from software adversary.
\end{itemize}
Security features have been added to the SoC to support the listed security objectives, including privilege-based access control to peripherals, writing locks on security-sensitive registers to prevent unprivileged code from compromising privilege level, and domain reset to flush sensitive information in cryptographic processors. Table~\ref{tab:secfea} demonstrates the security features for Key Manager, Keccak Message Authentication Code(KMAC), Hash-based Message Authentication Code(HMAC), One Time Programmable (OTP) memory controller, and Life Cycle (LC) Controller.
To perform security verification, we utilized the extracted security properties based on the threat model and security objectives. \textcolor{black}{ Since RTL descriptions of the SoCs are available to us, we craft the detailed security properties from the IP security specification and register checklists of the SoC.} These security properties span all the security features that were added to the SoC.

==> Table/table10.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.2}
\caption{Examples of misclassified security properties by ChatGPT for ${\cal{D}}_{val}$.}
%\vspace{0.1in}
\label{tab:gpt}
\begin{adjustbox}{width=0.90\textwidth,center}
\begin{tabular}{cl}
\hline \hline
\textbf{}             & \textbf{Generated Sentence}                                                                                                                                                                                                                                   \\ \hline \hline
\textbf{Property}     & \begin{tabular}[c]{@{}l@{}}The ADC is continually powered on.\end{tabular}                                                                               \\ \cline{2-2} 
\textbf{}             & \begin{tabular}[c]{@{}l@{}}It may be acceptable to disable the masking when using the AES cipher core for random number generation e.g. inside CSRNG.\end{tabular}                                                                 \\ \cline{2-2} 
\textbf{}             & \begin{tabular}[c]{@{}l@{}}In addition, they could potentially also be extracted when being transferred over the TL-UL bus interface.\end{tabular}                                      \\ \hline
\textbf{Non-property} & For encryption or if the mode is set to CFB, OFB or CTR, there is no such initial delay upon changing the key.                                                                                                                                                          \\ \cline{2-2} 
\textbf{}             & \begin{tabular}[c]{@{}l@{}}The AES unit cannot recover from such an error and needs to be reset.\end{tabular}                               \\ \cline{2-2} 
\textbf{}             & \begin{tabular}[c]{@{}l@{}}In this case, the AES unit never stalls and just overwrites previous output data, independent of whether it has been read or not.\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-0.1in}
\end{table*}

% \textbf{Property}     & \begin{tabular}[c]{@{}l@{}}Write access to a partition can be permanently locked when software determines it will no\\  longer make any updates to that partition.\end{tabular}                                                                               \\ \cline{2-2} 
% \textbf{}             & \begin{tabular}[c]{@{}l@{}}If a failure is encountered, the OTP controller will send out a fatal\_check\_error alert and \\ reset all of its hardware outputs to their defaults.\end{tabular}                                                                 \\ \cline{2-2} 
% \textbf{}             & \begin{tabular}[c]{@{}l@{}}Note however that only the life cycle controller has access to this partition, i.e., the Direct\\ Access Interface (DAI) cannot read nor write from/to the life cycle partition.\end{tabular}                                      \\ \hline
% \textbf{Non-property} & The OTP is a module that provides a device with one-time-programming functionality.                                                                                                                                                                           \\ \cline{2-2} 
% \textbf{}             & \begin{tabular}[c]{@{}l@{}}Since after power-up, these particular OTP contents are stored in flip flops and sourced to\\ the system. i.e., buffered partitions are NOT directly sourced from the OTP macro itself.\end{tabular}                               \\ \cline{2-2} 
% \textbf{}             & \begin{tabular}[c]{@{}l@{}}Generally speaking, the production life cycle of a device is split into 5 stages \\ “Manufacturing” -\textgreater “Calibration and Testing” -\textgreater “Provisioning” -\textgreater “Mission” -\textgreater “RMA”.\end{tabular} \\ \hline

==> Table/table9.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t!]
\renewcommand{\arraystretch}{1.2}
\caption{Examples for false-positives (FP) and false-negatives (FN) in security property generation.}
%\vspace{0.1in}
\label{tab:FPFN}
\begin{adjustbox}{width=0.90\textwidth,center}
\begin{tabular}{cl}
\hline \hline
\textbf{Category} & \textbf{Sentence}                                                                                                                                                                                                                                                                           \\ \hline \hline
\textbf{FP1}      & Note that interrupts are not provided, the latency of AES unit is such that they are little utility.                                                                                                                                                                                        \\ \hline
\textbf{FP2}      & How often FSM wakes up from ADC PD mode to take a sample, measured in always on clock cycles.                                                                                                                                                                                              \\ \hline
\textbf{FP3}      & Inside min=0, max=7: the value must be less than 8 to hit.                                                                                                                                                                                                                                  \\ \hline
\textbf{FN1}      & To this end, the processor has to set the SIDELOAD bit in CTRL\_SHADOWED to 1.                                                                                                                                                                                                              \\ \hline
\textbf{FN2}      & All ones should be written to adc\_intr\_status and filter\_status to ensure there are no spurious pending triggers.                                                                                                                                                                        \\ \hline
\textbf{FN3}      & \begin{tabular}[c]{@{}l@{}}If the next operation after a key switch is ECB or CBC decryption, the AES unit automatically initiates a key expansion \\ using the key schedule first (to generate the start key for decryption, actual data path remains idle during that phase)\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-0.1in}
\end{table*}

==> back.tex <==
Introduction

Hardware security validation is a crucial step in the hardware design process that helps ensure the security and trustworthiness of the design. It involves defining the threat model, identifying the relevant security properties, detecting any violations of those properties, and assessing the consequences to system security. Commercial design tools, such as Mentor Questa Secure Check, Cadence JasperGold Security Path Verification, and Tortuga Logic Radix, can be used to verify the security properties of a design. However, the effectiveness of these tools depends on the quality of the security properties provided to them. Therefore, the security properties of a design are a major element that provides resources for functional verification and security validation during any circuit development. However, generating appropriate security properties for each specific design can be a challenge. Traditional approaches often require the experience of developers and are limited to a small number of IPs, which can be time-consuming and lack robustness. To address this, we propose a technique that can systematically generate security properties, using descriptions of functionalities and operation behaviors from documents produced by major foundations, such as RSIC-V, MSP, and Arduino, and use these descriptions to generate security properties at the register level by correlating them with the operation of the RTL design. 

To bridge this gap, our goal is to provide a set of security properties for a SoC design or any processor by extracting essential information from the documentation and converting it into RTL-level assertions of the registers. By using this approach, we aim to systematically generate comprehensive and accurate security properties for each unique design.

Past work has shown in specialized domains like biomedicine that text can provide additional information over general-domain language models. By starting domain-specific pretraining from an existing general-domain language model (Figure 1 top). In this paper, we question this assumption. We observe that mixed-domain pretraining such as continual pretraining can be viewed as a form of transfer learning in itself, where the source domain is general text, such as newswire and the Web, and the target domain is specialized text such as biomedical papers. Based on the rich literature of multi-task learning and transfer learning [4, 13, 38, 59], successful transfer learning occurs when the target data is scarce and the source domain is highly relevant to the target one. For domains with abundant unlabeled text such as biomedicine, it is unclear that domain-specific pretraining can benefit by transfer from general domains. In fact, the majority of general domain text is substantively different from biomedical text, raising the prospect of negative transfer that actually hinders the target performance.

To bridge this gap, this paper presents an innovative method of contrastive pre-training to improve the language model representation for hardware specification extraction. As the main difference from the existing contrastive learning framework, we augment the datasets for RE tasks by randomly changing the words that do not affect the relation expression. Here, we hypothesize that the shortest dependency path (SDP) between two entities (Bunescu and Mooney, 2005) captures the required knowledge for the relation expression. We hence keep words on SDP fixed during the data augmentation. In addition, we utilize external knowledge bases to construct more data to make the learned representation generalize better, which is a method that is frequently used in distant supervision (Mintz et al., 2009; Peng et al., 2016).

Regenerate response

Natural Language Processing

Most of the processor designs have their dedicated documentation to describe the detailed functionalities and restrictions. Such information as register behaviors, operation privileges and functionality correctness can be utilized to generate security properties for each component of the design. Our goal is to develop a comprehensive framework to create security properties through documentation. We utilize the NLP language model to extract essential sentences from the documents and link them with their correlated module to transform them into semi assertions-based verification format.

In this task, we will aim to extract the register behavior information from the document through a machine learning language model. To do this, we will use the NLP language model to subtract the registers and behavior descriptions in the document that are directly related to these registers in RTL. The extracted sentences will be also used to enhance the model to target the desired security property elements more effectively by selecting sentences with more security-related information. Furthermore, we will use existing security properties from documents to train the model to search sentences with a condition check scenario. This process will be continuously repeated to achieve better efficiency for the NLP language model with more concentration and tuning, focusing on property-related contents. Fig. 15 shows the overall view of the documentation extraction framework.
